Joint Indoor Localization and Navigation of UAVs for Network Formation Control

In this paper, we propose a joint indoor localization and navigation algorithm to enable a swarm of unmanned aerial vehicles (UAVs) to deploy in a specific spatial formation in indoor environments. In the envisioned scenario, we consider a static user acting as a central unit whose main task is to acquire all the UAV measurements carrying position-dependent information and to estimate the UAV positions when there is no existing infrastructure for positioning. Subsequently, the user exploits the estimated positions as inputs for the navigation control with the aim of deploying the UAVs in a desired formation in space (formation shaping). The user plans the trajectory of each UAV in real time, guaranteeing a safe navigation in the presence of obstacles. The proposed algorithm guides the UAVs to their desired final locations with good accuracy.

==> defTagDet.tex <==
\newcommand{\rednote}[1] {{\color{red}$\blacktriangleright${#1}$\blacktriangleleft$}}
\newcommand{\blunote}[1] {{\color{blue}$\blacktriangleright${#1}$\blacktriangleleft$}}
\newcommand{\greennote}[1] {{\color{green}$\blacktriangleright${#1}$\blacktriangleleft$}}


\newcommand{\SNR} {{\mathsf{SNR}}}


\newcommand{\Real}[1]{\Re^{#1}}
\newcommand{\en} {E}
\newcommand{\td}[1] {\tilde{#1}}
\newcommand{\lt}[1] {{\td{\lambda}}_{#1}}
\newcommand{\bl}[1] {\text{\boldmath ${\lambda}$}_{#1}}
\newcommand{\blt}[1] {\text{\boldmath $\td{\lambda}$}_{#1}}
\newcommand{\vg}[1] {{\mbox{{\boldmath ${#1}$}}}}
\newcommand{\vgs}[2] {\vg{#1}_{#2}}

\newcommand{\PX}[1] {{\mathbb{P}}\left\{{#1}\right\}}
\newcommand{\EX}[1] {{\mathbb{E}}\left\{{#1}\right\}}
%\newcommand{\Var}[1] {{\mathbb{V}}\left\{{#1}\right\}}
\newcommand{\EXs}[2] {{\mathbb{E}}_{{#1}}\!\!\left\{{#2}\right\}}
\newcommand{\Var}[1] {{\text{Var}}\left ({#1}\right )}

\newcommand{\Tck} {\widetilde{T}_{\text{c}}^{(k)}}
\newcommand{\unierr}{\chi^2}
\newcommand{\sqrtunierr}{\chi}
\newcommand{\unierrsquare}{\chi^4}

\newcommand{\cl}{\mathpzc{c}}
\newcommand{\Pb} {P_{\mathrm{b}}}
\newcommand{\Pt} {P_{\mathrm{t}}}
\newcommand{\Rb} {R_{\mathrm{b}}}
\newcommand{\Ep} {E_{\mathrm{p}}}
\newcommand{\Et} {E_{\mathrm{t}}}
\newcommand{\Er} {E_{\mathrm{r}}}
\newcommand{\Ew} {E_{\mathrm{w}}}
\newcommand{\Eref} {E_{\mathrm{ref}}}
\newcommand{\Gref} {G_{\mathrm{ref}}}
\newcommand{\Tp} {T_{\mathrm{p}}}
\newcommand{\Td} {T_{\mathrm{d}}}
\newcommand{\fc} {f_{\mathrm{c}}}
\newcommand{\ts} {t_{\mathrm{s}}}
\newcommand{\Ta} {T_{\mathrm{a}}}
\newcommand{\Ti} {T_{\mathrm{i}}}
\newcommand{\Ted} {T_{\mathrm{ED}}}
\newcommand{\Np} {N_{\mathrm{p}}}
\newcommand{\Nd} {N_{\mathrm{d}}}
\newcommand{\Nps} {N_{\mathrm{ps}}}
\newcommand{\Npc} {N_{\mathrm{pc}}}
\newcommand{\tp} {\tau_{\mathrm{p}}}
\newcommand{\Es} {E_{\mathrm{s}}}
\newcommand{\Eb} {E_{\mathrm{b}}}
\newcommand{\Ts} {T_{\mathrm{s}}}
\newcommand{\Tf} {T_{\mathrm{f}}}
\newcommand{\Tc} {T_{\mathrm{c}}}
\newcommand{\Tb} {T_{\mathrm{b}}}
\newcommand{\Nc} {N_{\mathrm{c}}}
\newcommand{\Ns} {N_{\mathrm{s}}}
\newcommand{\Nsym} {N_{\mathrm{sym}}}
\newcommand{\Nt} {N_{\mathrm{t}}}
\newcommand{\Nr} {N_{\mathrm{r}}}
\newcommand{\tint} {T_{\mathrm{int}}}
\newcommand{\TX}[1] {{\mathbb{T}}\left [{#1}\right ]}
\newcommand{\Prob}[1] {\mathrm{P}\left\{{#1}\right\}}
\newcommand{\Q}[1] {Q \left ( #1 \right )}
\newcommand{\Nch} {N_{\mathrm{ch}}}
\newcommand{\Lp} {L_{\mathrm{p}}}
\newcommand{\dref} {d_{\mathrm{ref}}}
\newcommand{\wref} {w_{\mathrm{ref}}}
\newcommand{\Wref} {W_{\mathrm{ref}}}
\newcommand{\Href} {H_{\mathrm{ref}}}
\newcommand{\ZA} {Z_{\mathrm{A}}}
\newcommand{\hmf} {h_{\mathrm{MF}}}
\newcommand{\Tob} {T_{\mathrm{ob}}}
\newcommand{\taup} {\tau_{\mathrm{f}}}
\newcommand{\etaup} {\hat{\tau}_{\mathrm{f}}}
\newcommand{\taud} {{\tau_{\mathrm{d}}}}
\newcommand{\etaud} {\hat{\tau}_{\mathrm{d}}}
\newcommand{\toa} {\tau}
\newcommand{\etoa} {\hat{\tau}}
\newcommand{\Beff} {B_{\mathrm{eff}}}
\newcommand{\Gr} {G_{\mathrm{r}}}
\newcommand{\Gt} {G_{\mathrm{t}}}
\newcommand{\Pric} {P_{\mathrm{r}}}
\newcommand{\thetar} {{\bf \Theta}_{\mathrm{r}}}
\newcommand{\thetat} {{\bf \Theta}_{\mathrm{t}}}

\newcommand{\Nspan}{N_{\mathrm{span}}}

\newcommand{\floor}[1] {f \left ({#1} \right )}
\newcommand{\Ntag}{N_{\mathrm{tag}}}
\newcommand{\Nbin}{N_{\mathrm{bin}}}
\newcommand{\Nce}{N_{\mathrm{ce}}}

\newcommand{\sreader}{s_{\mathrm{reader}}}
\newcommand{\stag}{s_{\mathrm{tag}}}
\newcommand{\rreader}{r_{\mathrm{reader}}}
\newcommand{\rtag}{r_{\mathrm{tag}}}
\newcommand{\pI}{p_{\mathrm{I}}}
\newcommand{\pII}{p_{\mathrm{II}}}
\newcommand{\wI}{w_{\mathrm{I}}}
\newcommand{\wII}{w_{\mathrm{II}}}
\newcommand{\gammaI}{\gamma_{\mathrm{I}}}
\newcommand{\gammaII}{\gamma_{\mathrm{II}}}
\newcommand{\Ec} {E_{\mathrm{c}}}

\newcommand{\xho} {x^{(\mathcal{H}_{0})}(t)}
\newcommand{\xhone} {x^{(\mathcal{H}_{1})}(t)}
\newcommand{\xh} {x^{(\mathcal{H})}(t)}

\newcommand{\xhoi} {x_{i}^{(\mathcal{H}_{0})}\,}
\newcommand{\xhonei} {x_{i}^{(\mathcal{H}_{1})}\,}

\newcommand{\Ho}{\mathcal{H}_{0}}
\newcommand{\Hone}{\mathcal{H}_{1}}
\newcommand{\Nmf}{N_\mathrm{MF}}

\newcommand{\pd}{P_{\text{D}}}
\newcommand{\pds}{P_{\text{D}}^{*}}
\newcommand{\pfa}{P_{\text{FA}}}
\newcommand{\pfas}{P_{\text{FA}}^{\star}}
\newcommand{\pfr}{P_{\text{FR}}}
\newcommand{\pfar}{P_{\text{FR}}^{\star}}
\newcommand{\pscr}{P_{\text{SC}}^{\star}}


\def\dsp{\displaystyle}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\def\erfc{{\text{erfc}}}
\def\erf{{\text{erf}}}
\def\inve{{\text{inverfc}}}
\def\teq{\triangleq}
\def\bs{$\blacksquare$}
